PINPOINT: Efficient and Effective Resource Isolation for Mobile Security and Privacy

Virtualization is frequently used to isolate untrusted processes and control their access to sensitive resources. However, isolation usually carries a price in terms of less resource sharing and reduced inter-process communication. In an open architecture such as Android, this price and its impact on performance, usability, and transparency must be carefully considered. Although previous efforts in developing general-purpose isolation solutions have shown that some of these negative side effects can be mitigated, doing so involves overcoming significant design challenges by incorporating numerous additional platform complexities not directly related to improved security. Thus, the general purpose solutions become inefficient and burdensome if the end-user has only specific security goals. In this paper, we present PINPOINT, a resource isolation strategy that forgoes general-purpose solutions in favor of a "building block" approach that addresses specific end-user security goals. PINPOINT embodies the concept of Linux Namespace lightweight isolation, but does so in the Android Framework by guiding the security designer towards isolation points that are contextually close to the resource(s) that need to be isolated. This strategy allows the rest of the Framework to function fully as intended, transparently. We demonstrate our strategy with a case study on Android System Services, and show four applications of PINPOINTed system services functioning with unmodified market apps. Our evaluation results show that practical security and privacy advantages can be gained using our approach, without inducing the problematic side-effects that other general-purpose designs must address.

==> background.tex <==
\section{Linux Namespaces}
\label{sec:namespaces}

Before enumerating the key traits and values of the Linux Namespace concept in Section \ref{subsec:traits}, we first provide a brief technical background for readers not completely familiar.

\subsection{Background}
\label{subsec:background}

Since their introduction to the mainstream Linux kernel beginning in 2002, Linux Namespaces have enabled a form of kernel-enforced process-level virtualization, useful for isolating specific resources within a single instance of the operating system. In contrast to hypervisor-based approaches, Namespaces represent a lightweight, ``only what's needed,'' approach to virtualizing various aspects of a process's environment. This container architecture is arguably more scalable and efficient than full virtualization solutions \cite{Strauss:2013:FCC:2492102.2492107} \cite{Soltesz:2007:COS:1272996.1273025}. Practical uses for Namespaces include resource sharing \cite{Biederman:2006:Namespaces:OLS}, checkpointing/migration, \cite{Bhattiprolu:2008:VSC:1400097.1400109} vulnerability containment, and binary isolation \cite{Jain:2014:PTO:2592798.2592811}.

Simply put, namespaces allow different objects to have the same name. For example, the objects ``server1'' and ``server2'' could both have the name ``hostname'' in different namespaces. In Linux, the original motivation for including namespace support were the needs of virtual private servers (VPS) and application checkpoint and restart (ACR) \cite{Bhattiprolu:2008:VSC:1400097.1400109}. Six namespaces make up the current Linux implementation discussed here: \textit{mount}, \textit{hostinfo}, \textit{System V IPC}, \textit{pid}, \textit{network}, and \textit{userid}. Each of these orthogonal namespaces address a different aspect of the system which can be virtualized for particular applications. They can be used in any combination or individually. Finally, while the main feature of namespaces can be described as lightweight virtualization, namespaces also represent a form of isolation since access to namespaces is controlled by the Linux kernel. Creation and management of Linux namespaces done through privileged system calls.

%Namespaces are created and managed by way of three privileged system calls: \texttt{clone()}, \texttt{unshare()} and \texttt{setns()}. \texttt{clone()} forks a new process into a new namespace, while \texttt{unshare()} and \texttt{setns()} allow the calling process to leave and join other namespaces, respectively. Configuration of each new namespace is specified using some twenty-two different \texttt{CLONE\_*} flags to identify the type, and how the caller's execution context is to be shared.

Implementation of namespaces within the Linux kernel is accomplished by way of a proxy structure of pointers, \texttt{nsproxy}. As namespace support was added to the kernel, system calls that interact with namespace objects were rewritten to use this proxy rather than referencing objects directly. Hence, one process's \texttt{nsproxy} may point to different objects as compared with another's. From these two processes' point of view, they are using the exact same name to reference the object, but are given back different objects. The object returned is determined by the state of \texttt{nsproxy}, which is out of the process's control. In a sense, each process is isolated from other objects with the same name in different namespaces. This isolation is immutable because the redirection is enforced by the kernel, within the trusted computing base (TCB).

%To illustrate this implementation, we use the \textit{hostinfo}, or \textit{UTS}\footnote{This name derives from Unix Timesharing System, abbreviated \texttt{uts} in the source code of many Unix-like operating systems.} namespace as an example. UTS namespaces isolate two system identifiers returned by the \texttt{uname()} system call, namely \texttt{nodename} and \texttt{domainname}.  Prior to kernel version 2.6.19, these values were returned by reading them from global kernel parameters, \texttt{system\_utsname.nodename} and \texttt{system\_utsname.domainname}, respectively. As a result, these objects had the same values for all processes. Beginning with the introduction of UTS namespace support in kernel version 2.6.19, these values are read from a private kernel data structure, \texttt{nsproxy}. One member of \texttt{nsproxy} is a pointer to a structure containing UTS namespace objects such as \texttt{nodename} and \texttt{domainname}. Processes that have all the same namespaces share \texttt{nsproxy}, but it is copied and its pointers changed when one of the namespaces is cloned or unshared. In this way, the \texttt{nsproxy} structure enables the kernel to hold different objects (i.e., values) referenced with the same name (e.g., \texttt{nodename}, \texttt{domainname}) by different processes.

In userspace, namespace support adds a set of symbolic links in \path{/proc/<pid>/ns}, one for each namespace supported. These links act as ``handles'' for processes to use to interact with the namespaces. For example, the handles can be compared across two processes to determine if they belong to the same namespace. Also, by passing a file descriptor for one of these links to \texttt{setns()}, a privileged process may join the namespace \cite{Kerrick2013}.

\subsection{Namespace Traits and Their Value to Our Work}
\label{subsec:traits}

%With a modified Linux kernel at its heart, and resource constraints that may preclude full virtualization, Android is a great candidate to take advantage of the benefits of Linux Namespaces.  In fact, recent versions supporting multiple users and restricted profiles leverage mount namespaces to isolate each user's external storage \cite{ExtStorage}. It is likely that future Android releases will make further use of these facilities.

As mentioned earlier, our objective is not to isolate Framework objects using Linux Namespaces themselves, but to develop a specific virtualization and isolation architecture that reflects the same high-level benefits as Linux Namespaces. To do this, we conducted a systematic analysis to extract a list of key traits and link these to specific benefits that our architecture should realize. A summary of the following analysis is found in Table \ref{table:traits}.

\newcounter{val}

\refstepcounter{val}\label{val:perproc}
\subsubsection{Namespaces virtualize and isolate specific resources on a per-process basis} Namespaces provide a level of abstraction that wraps certain resources, allowing them to appear to be dedicated to a particular process rather than globally shared \cite{Kerrick2013}\cite{WikiNamespace}. These virtual resources are isolated because the kernel controls which processes can join or leave a namespace.

\textit{Value to our work:} The fine granularity of namespace isolation allows each process to be placed in a tailored virtual environment. Processes spawned by untrusted applications can be presented with a surrogate or subset of sensitive, otherwise global resource(s), thus making it impossible for the application to misuse the resource(s). This can be done permanently for some applications or temporarily while trust is established during testing and debugging \cite{Rosen2014}.

\refstepcounter{val}\label{val:resource} 
\subsubsection{Namespaces are resource-centric} When there is a specific resource that must be isolated, namespaces are able to address the isolation directly, unlike coarse-grained approaches such as platform virtualization.

\textit{Value to our work:} Mobile device users are concerned with their privacy and personal data, and typically think in terms of these high-level semantics rather than trying to understand the details of why an application needs certain permissions and how granting that permission could negatively affect them. At the same time, users want their applications to work smoothly and provide the functionality they desire (but no more). By isolating resources using semantics similar to the user's point of view, namespaces relieve the user from having to understand low-level access control mechanisms and the permission-to-resource mappings. This translates to a high level of usability, not just for the user's configuration of namespaces, but also for the platform as a whole. Moreover, because Android is based on an open architecture that facilitates and depends on a high level of interaction among apps, isolating only certain critical resources preserves other functionality without having to implement complex workarounds or inconveniencing the user.

\refstepcounter{val}\label{val:efficient} 
\subsubsection{Namespaces are efficient} Linux Namespaces share a single kernel and operating system instance \cite{Strauss:2013:FCC:2492102.2492107}\cite{Rosen2014}. As a result, isolation of a specific resource can be achieved with high efficiency, and overall performance levels are nearly identical those without any isolation \cite{Strauss:2013:FCC:2492102.2492107}\cite{Soltesz:2007:COS:1272996.1273025}\cite{Bhattiprolu:2008:VSC:1400097.1400109}\cite{Biederman:2006:Namespaces:OLS}. Unlike isolation based on platform or application virtualization, there is no extra startup time for a namespace \cite{Strauss:2013:FCC:2492102.2492107}.

\textit{Value to our work:} By applying the namespace concept to high level semantics of the Android Framework, we carry forward the efficiency advantages of the namespace concept. Just as Linux Namespaces share a single kernel and OS instance, our namespaces share a single Framework and runtime instance.  In the constrained environment of a mobile device, this is an extremely important trait.

\refstepcounter{val}\label{val:share} 
\subsubsection{Namespaces share by default} Namespaces provide strong isolation of certain resources while permitting sharing of others \cite{Soltesz:2007:COS:1272996.1273025}\cite{Bhattiprolu:2008:VSC:1400097.1400109}\cite{Biederman:2006:Namespaces:OLS} . This contrasts with isolation based on coarse-grained platform or application virtualization where communication among processes in different virtual machines is difficult, and may require modifications to either applications or the virtual machines themselves.

\textit{Value to our work:} Android is a platform designed around the fact that apps are closely related and must communicate in order to provide the best usability and efficiency. In fact, most of the Android system itself uses these same channels for system-app and system-system communications. Isolating resources by way of fine-grained namespace virtualization at the Framework level preserves continued sharing of resources unrelated to the isolated resource. Coarse-grained virtualization breaks many shared resources that have nothing to do with the isolated resource.

\refstepcounter{val}\label{val:trans} 
\subsubsection{Namespaces are transparent} Namespaces are transparent to the host system, as well as to the applications inside them \cite{Strauss:2013:FCC:2492102.2492107}\cite{Bhattiprolu:2008:VSC:1400097.1400109}. This means that processes running in a namespace appear as normal processes to the host system, and the host system appears normal to an application. The host system retains the full ability to monitor, analyze, and directly control all processes, and the application need not be modified to run in the namespace. This is not always the case with other forms of virtualization such as platform and application virtualization. In the former, the host system loses visibility and control over the individual processes running within the VM, and in the latter, the application may need to be modified to account for unrepresented resources.

\textit{Value to our work:} By applying the namespace concept to the Framework, a single Android system and kernel retains full control over all applications, and apps do not need modifications to work properly.

\refstepcounter{val}\label{val:footprint} 
\subsubsection{Namespaces have a small footprint} Unlike many forms of platform and application visualization, namespaces do not require persistent files or large binaries, and have a small kernel footprint, making them lightweight \cite{Strauss:2013:FCC:2492102.2492107}\cite{Soltesz:2007:COS:1272996.1273025}\cite{Bhattiprolu:2008:VSC:1400097.1400109}\cite{Biederman:2006:Namespaces:OLS}.

\textit{Value to our work:} Mobile devices are resource-constrained and most users will become very impatient with security features that consume storage or negatively impact performance.  By addressing only a specific, high-level resource, namespaces applied to the Framework can be implemented with relatively few modifications to the Android system, and only a small amount of memory consumed.  This results in nearly zero impact on storage resources and device performance. In addition, since mobile devices are usually subject to disadvantaged or expensive communication links, the small footprint opens the possibility of practical over-the-air (OTA) configuration or update.

\begin{table*}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Summary of Namespace Traits and Their Value to Android Security}
\label{table:traits}
\centering
\begin{tabular}{c||c}
\hline
\bfseries Namespace Trait & \bfseries Value to Android Security\\
\hline\hline
Fine-grained isolation of specific resources & Tailored isolation environment for each application, addressing specific threat and/or user goal\\
\hline
Resource-centric isolation & Match user perspective on security; increase usability; simplicity\\
\hline
High efficiency & Negligible performance impact; design simplicity\\
\hline
Share-by-default & Preserve open system design; avoid breaking things unrelated to the isolated resource\\
\hline
Transparent to host and apps & System retains control over apps; apps run unmodified\\
\hline
Small footprint (files, memory) & Little impact on performance \& resources; OTA updates\\
\end{tabular}
\end{table*}


==> config.tex <==
\subsection{PINPOINTing Apps}
\label{subsec:user_config}

In our current prototype, user-friendly assignment of apps to namespaces is done via our specialized launcher, \textit{SecureLauncher}. This launcher, shown at \ding{174} in Figure \ref{fig:design}, has the privilege to modify entries in the policy definition file.

%\texttt{EERIMS} configuration is loaded from \texttt{nspolicy} file. As discussed, \texttt{servicemanager} would decide on which instance of virtualized services to return for a request from an app based on configurations in this file. Our aim is to make this design highly configurable, transparent to the app as well as native system and seamless in user experience of Android. Similar to \texttt{Intent Firewall}, we wanted to enable hot swap for all the configurations of \texttt{EERIMS}. Any change to the file, \texttt{nspolicy}, will be instantly reflected in the system. Theoretically, there are two kinds of configuration in this solution: First, one that chooses which of the virtualized services that will honor a given request and second, one that would determine a given service's properties. For example, a request for location update can be routed to one among many virtualized location services based on one configuration and the service working on the reply can add different amount of noise to the real location based on value passed to \texttt{LocationFudger} from second configuration. To show how effortless these changes could be modified, we prototyped an Android Launcher.

Though every app could have its own unique assignments, a great user experience is possible when we have groups of apps with a common set of assignments. Launcher is a logical and intuitive way to create these assignment ``containers'' because of its inherent nature of grouping apps using constructs such as homescreens, folders, etc. For example, common assignment configurations could include \textit{Sensitive Apps}, \textit{Trusted Apps}, \textit{Untrusted Apps}, etc. Based on this concept, we built containers, represented by homescreens, with predefined combinations of namespaces defined for the group of apps in the container.

For simplicity, each namespace in a container is preconfigured through a list of settings. Drag and drop of apps between homescreens will update the namespace assignment(s) of the app in the policy definition file, \texttt{nspolicy}. For example, if a user wants his online food delivery app to stop receiving an accurate location, as shown in Figure \ref{fig:config}, moving the app from one screen (\ref{fig:configwithone}) to another (\ref{fig:configwithtwo}) will automatically update the app's namespace assignments in the policy file. 

\begin{figure}[!t]
  \centering
  \subfigure[\texttt{SecureLauncher} showing app icon in container 1. User may drag-and-drop app icon as shown by arrow to assign app to different namespace(s).]{\label{fig:configwithone}
    \includegraphics[width=0.2\textwidth]{Figs/Launcher1-arrow.png}}
  \qquad
  \subfigure[\texttt{SecureLauncher} showing app icon moved to container 2 following drag-and-drop operation. \texttt{SecureLauncher} also updates the policy file following this operation.]{\label{fig:configwithtwo}
    \includegraphics[width=0.2\textwidth]{Figs/Launcher2.png}}
  \caption{Using \texttt{SecureLauncher} to configure app namespace assignments.}
  \label{fig:config}
\end{figure}


==> space.tex <==


%With this in mind, we are motivated to find less general alternate approaches that are still highly effective for containing specific threats or classes of threats and without significant side effects. In order to evaluate alternatives, consider the following qualitative measures of effectiveness and efficiency:

%With this in mind, we strive to map out the isolation design space such that we can find alternate solutions that are still effective for specific threats or classes of threats, while remaining transparent to developers, negligible in their performance impacts, free of complex changes to the system, and low-cost to the end-user in terms of usability and convenience. As we traverse the design space, we will consider the following qualitative aspects as our measures of merit for each design alternative:

%\textit{Effectiveness:}
%\begin{enumerate}
%  \item \textit{Range of threats}: does the design address a wide range and variety of threats?
%  \item \textit{Adequacy}: is the design adequate in containing the threats it is intended to address?
%  \item \textit{Isolation ``size''}: is the isolation comprehensive, resulting in a small attack surface (few things shared)?
%\end{enumerate}

%Together, these measures relate to the notion of \textit{effectiveness}, while an aggregation of the following contribute to \textit{efficiency}:

%\textit{Efficiency:}
%\begin{enumerate}
%  \item \textit{Complexity}: does the design require far-reaching or complex modifications to the Android system in order to restore basic platform functionality or compensate for loss of end-user usability/convenience?
%  \item \textit{Transparency}: does the design require special considerations on the part of the application developer, i.e., do apps need to be modified to function?
%  \item \textit{Performance}: does the design have a significant impact on overall device performance in terms of start-up, application launch, user interface response, etc.?
%  \item \textit{Usability and convenience}: will the end-user face significant concessions in terms of usability and/or convenience in order to realize their security goals?
%\end{enumerate}

%\subsection{Tradespace}

%Consider the simplified Android architecture diagram of Figure \ref{fig:android_arch}. Here we see that all applications and high-level system services share a single runtime, with inter-app communication facilitated by \textit{Binder}, Android's lightweight IPC subsystem \cite{Binder}. Now consider the situation where we don't trust App 2 and wish to isolate it in some way. This diagram now represents our tradespace, where we can consider the overall ramifications of different approaches to isolating App 2, in terms of the seven qualitative measures of merit introduced above.

% This figure uses numbers in circles to facilitate references from within the text. In the text, \ding{172} will be rendered as a 1 in a circle, \ding{173} as a 2, etc.

%\begin{figure}[!t]
%\centering
%\includegraphics[width=3in]{Figs/android_arch.pdf}
%\caption{Simplified Android architecture.}
%\label{fig:android_arch}
%\end{figure}

%First, we could totally isolate it by running it on an entirely different instance of the kernel and operating system (i.e., ``dual boot''), where the only thing shared between the two apps is the device hardware (Figure \ref{fig:android_arch}, location \ding{172}). Using a mechanism like the open source \textit{BootManager} project \cite{BootManager}, this approach provides a strong isolation between our untrusted app, App 1 and the system services on the OS instance we wish to protect. However, this very strong isolation comes with a very high price. Usability and convenience suffer greatly since switching between apps involves a full reboot, and interactive sharing of data and resources becomes impossible. Also, as is common in Android, App 2 may depend on components of App 1 for full functionality, requiring separate copies of App 1 to be installed in both boot partitions. On the other hand, the isolation is very strong, and even if App 2 is able to exploit kernel vulnerabilities, it cannot escape its isolation and affect App 1. 

%Inserting a virtualization layer at location \ding{172} to enable simultaneous virtual machines (VM) is another approach that recent work has shown possible \cite{Dall:2014:KDI:2541940.2541946}. This is the ``bare metal'' or Type 1 hypervisor design that would increase convenience somewhat by precluding the need for full reboots to switch between apps. Isolation with a native hypervisor is still very comprehensive, presenting App 2 with a very small attack surface. However, many of the sharing and open communication tenets of the Android design are still broken and would require a significant amount of added complexity to restore.

%If we instead allow the isolated app to share both the hardware, kernel and some native Android operating system resources with the trusted app (Figure \ref{fig:android_arch}, location \ding{173}), one major aspect of usability improves somewhat. Similar to Type 2 hypervisor architectures, the user no longer has to reboot the device to switch apps. While the shared kernel and native processes represent additional attack surfaces (App 2 can now use a kernel vulnerability to escape its isolation and attack App 1), it enables low-level sharing of raw resources and communication channels, and the design is still general enough to address a wide variety of common threats. Unfortunately, Android fundamentally assumes a common runtime, and breaking this assumption introduces many difficulties. To address these difficulties, one must undertake challenging and complex side projects, such as those described in \cite{wu2014airbag} and \cite{Dall:2012:DIE:2324876.2324877}, which both use different variations of this approach to isolation.

%Another possibility would be to allow the apps to share the same hardware, kernel and runtime, but not share the entirety of a frequently-misused subsystem such as Binder (Figure \ref{fig:android_arch}, location \ding{174}). From results described in \cite{Bugiel:2011:PLD:2046614.2046624}, where this approach was taken, we see that although the effectiveness is limited to threats promulgated through IPC, nasty system problems (and corrective complexity) that come with isolating the Android runtime have been avoided. Usability and convenience also benefit, since an isolated IPC subsystem likely has much less negative effect on performance than does concurrent instances of the Android runtime environment. App 2's attack surface is also greater, since it now has the opportunity to exploit vulnerabilities in aspects of the framework other than IPC. Again, whether this was a prudent trade-off depends on the end-user's expectations and the threats they need addressed.

%\begin{table*}[!t]
%\renewcommand{\arraystretch}{1.3}
%\caption{Summary of Isolation Design Alternatives}
%\label{table:alternatives}
%\centering
%\begin{tabular}{c||c||c||c||c||c||c||c}
%\hline
%\bfseries Design & \bfseries Range of threats & \bfseries Adequate & \bfseries Isolation size & \bfseries Complexity & \bfseries Transparent & \bfseries Performance & \bfseries Usability/convenience \\
%\hline\hline
%Dual-boot & Most & Yes & Large & High & Yes & Excellent & Low\\
%\hline
%Type 1 hypervisor & Most & Yes & Large & High & Yes & Excellent & Low+\\
%\hline
%Type 2 hypervisor & Many & Yes & Medium & Medium & Yes & Good & Medium\\
%\hline
%Isolated IPC & Few & Yes & Small & Low & Yes & Excellent & Good\\
%\end{tabular}
%\end{table*}

%As can be seen by the design alternative summary in Table \ref{table:alternatives}, it's clear by now that things like complexity, usability, and the range of threats addressed appear to be strongly correlated to how much of the system is shared by the isolated app and how much is part of the isolation itself (isolation size).  If large portions of the system are part of the isolation (i.e., not much is shared between trusted and untrusted apps), many threats are addressed, but usability drops off, countered only by a commensurate increase in complexity to fix things. Conversely, as more system components are shared among all apps, fewer threats are addressed, but usability suffers less and fewer complex system modifications are required to compensate. At this level of analysis, all designs are assumed to be adequate in addressing the threats they were designed to address, and transparent to apps (i.e., apps can run unmodified without crashing). Thus, we can summarize the more interesting aspects of the design tradespace by noting a few apparent correlations among several of our measures of merit:

%\begin{enumerate}
%  \item Range of threats increases as isolation size increases (i.e., the attack surface decreases).
%  \item Complexity increases (i.e., having to fix things that the isolation broke) as isolation size increases.
%  \item Usability and convenience decreases as isolation size increases.
%\end{enumerate}

%Thus, when the security goal is to address a specific threat or threats, the best solution would be one that isolates only what's necessary and nothing more. In this way, threats are addressed without sacrificing any more usability than necessary and without increasing ancillary complexity (that which is not directly related to the security goals) any more than necessary. In \cite{Bugiel:2011:PLD:2046614.2046624}, this mindset is what allows their approach to isolating IPC to be termed ``lightweight.'' In our work however, we consider this as a more general design principle that is potentially applicable to many different objects throughout the Android Framework, not just IPC. As such, we now more clearly define our concept in general terms.

